Objective barriers to the transport of dynamically active vector fields

We derive a theory for material surfaces that maximally inhibit the diffusive transport of a dynamically active vector field, such as the linear momentum, the angular momentum or the vorticity, in general fluid flows. These special material surfaces (\emph{Lagrangian active barriers}) provide physics-based, observer-independent boundaries of dynamically active coherent structures. We find that Lagrangian active barriers evolve from invariant surfaces of an associated steady and incompressible \emph{barrier equation}, whose right-hand side is the time-averaged pullback of the viscous stress terms in the evolution equation for the dynamically active vector field. Instantaneous limits of these barriers mark objective \emph{Eulerian active barriers} to the short-term diffusive transport of the dynamically active vector field. We obtain that in unsteady Beltrami flows, Lagrangian and Eulerian active barriers coincide exactly with purely advective transport barriers bounding observed coherent structures. In more general flows, active barriers can be identified by applying Lagrangian coherent structure (LCS) diagnostics, such as the finite-time Lyapunov exponent and the polar rotation angle, to the appropriate active barrier equation. In comparison to their passive counterparts, these \emph{active LCS diagnostics} require no significant fluid particle separation and hence provide substantially higher-resolved Lagrangian and Eulerian coherent structure boundaries from temporally shorter velocity data sets. We illustrate these results and their physical interpretation on two-dimensional, homogeneous, isotropic turbulence and on a three-dimensional turbulent channel flow.

==> channelflow.tex <==
% ==============================================================================
% ==============================================================================
\subsection{Three-dimensional low-Reynolds number channel flow\label{subsec:channelflow}}

We consider now the incompressible three-dimensional turbulent flow of a Newtonian
fluid in a doubly periodic channel, which serves as well-known flow scenario to discuss, for the first 
time, active barriers in a three-dimensional turbulent flow.


The results presented in the following rely
upon a database of flow snapshots obtained via DNS. {\color{red} XXX Check if acronym has been defined before}
The DNS code employed in the present study is based on the mixed-discretization parallel 
solver of the incompressible Navier--Stokes equations in the wall-normal
velocity and vorticity formulation developed by Luchini \& Quadrio
(2006). The equations of motions are discretized via a Fourier--Galerkin
approach along the two statistically homogenous streamwise $\left(x\right)$ and
spanwise $\left(z\right)$ directions. Fourth-order compact finite differences
(Lele 1992) based on a five-point computational stencil are adopted
in the wall-normal direction $\left(y\right)$.


The governing equations are integrated forward in time at constant
power input {\color{red} (Hasegawa et al. 2014)} with a partially-implicit approach, combining the
three-step low-storage Runge\textendash Kutta (RK3) scheme with the
implicit Crank\textendash Nicolson scheme for the viscous terms. The
friction Reynolds number is $Re_{\tau}=u_{\tau}h/\nu=200$, based
on the friction velocity $u_{\tau}$, the channel half height $h$
and the kinematic viscosity $\nu$, which corresponds to a bulk Reynolds
number $Re_{b}=U_{b}h/\nu=3177$, where $U_{b}$ is the bulk velocity. 
The computational domain is $L_{x}=4\pi h$ long
and $L_{z}=2\pi h$ wide. The number of Fourier modes is 256 both
in the streamwise and spanwise direction; the number of points in
the wall-normal direction is 256, unevenly spaced in order to decrease
the grid size near the walls. The corresponding spatial resolution
in the homogeneous directions is $\Delta x^{+}=9.8$ and $\Delta z^{+}=4.9$ 
(without accounting for the additional modes required for dealiasing
according to the 3/2 rule); the 
wall-normal resolution increases from $\Delta y^{+}=0.4$ near the walls to 
$\Delta y^{+}=2.6$ at the centreline,
while the temporal resolution is kept constant at $\Delta t=0.005 h/U_b$, corresponding to $\Delta t^{+}=0.063$.
The superscript $+$ denotes nondimensionalization in viscous units,
i.e. with $u_{\tau}$ and $\nu$. At each DNS timestep and thus with the same 
temporal resolution, a three-dimensional flow snapshot is stored for a total 
of 1500 snapshots. The 750$^\mathrm{th}$ snapshot in the series is stored at time
$t=0$. This is the instant at which the instantaneous barriers are computed. The last 750 snapshots are utilised for the computation 
of the active barriers and classic forward FTLE, while the first 750 ones are used 
for calculating the classic backward FTLE. The integration time for the Lagrangian calculations
has been chosen based on pair dispersion statistics of Lagrangian tracers {\color{red} (see, for instance, Pitton et al.
2012)}. The averaging time for the 
bulk flow statistics is  8100 $U_b / h$. In the following, 
all quantities are nondimensionalized using  $U_{b}$ and $h$ unless stated
otherwise.


The active barriers are computed within a two-step procedure. First, the active 
barrier field $\mathbf{b}_{t_0}^{t_1}\left(\mathbf{x}_0\right)$, appearing at the right-hand 
side of the barrier equation {$\color{red} (20)$}, is computed. Then, the barrier 
ODE is solved and visualised through FTLE and PRA diagnostics. 

\begin{figure}
  \centering
  \includegraphics[width=0.9\textwidth]{./Figures/Cartoons/seed.pdf}
  \caption{Sketch of the computational molecule utilised for the computation of the active barrier field $\mathbf{b}_{t_0}^{t_1}$. The large circle denotes the Lagrangian tracer at the center of the molecule, where the vector field  $\mathbf{h}_{vis}$ is computed. The cross denotes the further six tracers utilised to compute $\nabla\mathbf{F}_{t_0}^{t_1}$. }
  \label{fig:seed}
\end{figure}
For instantaneous barriers, the barrier field is readily computed from the velocity field data
as $\mathbf{b}_{t}^{t}=\mathbf{h}_{vis}$. Differentiation of the velocity field is  performed with 
the same discrete operators used during DNS. For material barriers, $\mathbf{b}_{t_0}^{t_1}\left(\mathbf{x}_0\right)$ is obtained as temporal average of 
 $\left(\mathbf{F}_{t_0}^{t_1}\right)^\ast \mathbf{h}_{vis}$. In this case, the vector field $\mathbf{b}_{t_0}^{t_1}\left(\mathbf{x}_0\right)$ is discretised 
on a Cartesian grid similar to the one used for the velocity field; the only difference being that the
number of collocation points along the $x$- and $z$-directions is increased to 
384 via Fourier interpolation. At time $t_0$, a set of tracers is seeded in the 
neighbourhood of each point $\mathbf{x}_0$ at which $\mathbf{b}_{t_0}^{t_1}\left(\mathbf{x}_0\right)$ 
needs to be computed. Each set (see figure~\ref{fig:seed}) is composed by  7 tracers. The central 
tracer is exactly located at $\mathbf{x}_0$ and is the only one along which the vector field $\mathbf{h}_{vis}$ is also computed.
The other tracers are shifted by $\epsilon_i$ along the positive and negative $i$th spatial direction and are
utilised to compute $\nabla \mathbf{F}_{t_0}^{t_1}\left(\mathbf{x}_0\right)$ with second-order central finite differences. 
The shift $\epsilon_i$ is defined as $1/100$ of the minimum grid spacing along the $i$th spatial direction. 
A total of $2.64\times 10^8$ particles are seeded into the flow. The evolving positions of these
tracers, which are images of their initial positions under the flow
map $\mathbf{F}_{t_0}^{t_1}$, are advanced in time by integrating the
$\mathbf{u}$ field with a third-order four-stage Runge--Kutta algorithm. The vector fields $\mathbf{u}$ and 
$\mathbf{h}_{vis}$ required at the intermediate stages are obtained via linear interpolation of two consecutive flow snapshots 
and are evaluated at the particle position through a sixth-order, three-dimensional
Lagrangian interpolation {\color{red} (van Hinsberg et al. 2012, Pitton et al.
2012)} of the underlying vector field, which reduces to fourth-order
only between the wall and the first grid point above it. 


Once the (material or instantaneous) barrier field is available, its active flow map $\mathbf{F}_{t_0,t_1}^{s}$
is computed by solving the steady barrier ODE up to a value $s$ of 31.0 and 0.62
 for the momentum and vorticity barriers respectively. The actual value of 
$s$ does not significantly affect the results, provided it is large enough for
the computed field lines to capture the behaviour of the underlying barrier field and small enough
to avoid accumulation of the integration error, the latter being a circumstance that we have 
never observed for the present parameter choice. The effect of changing the parameter $s_{\mathrm{max}}$ is shown in the
additional material {\color{red} \textsf{Movie 1.mov}} and {\color{red} \textsf{Movie 2.mov}}
for instantaneous momentum and vorticity barriers respectively. The seeds for the flow map are
arranged in a Cartesian grid identical to the one of the active barrier field for three-dimensional  
computations of aFTLE/aPRA diagnostics, while the spatial resolution is increased by a factor 6 along when only two-dimensional
slices are computed. The comparison between the two resolutions has been utilised to verify the grid-independence of the results. The aFTLE and aPRA diagnostics are then computed according to equations {\color{red} (68)} 
and {\color{red} (74)} respectively. 

% ==============================================================================
% ==============================================================================
\subsubsection{Instantaneous barriers to active transport} \label{sec:i3d}

Instantaneous aFTLE and aPRA are presented for $t=0$ in figures \ref{fig:channel_iFTLE} and 
\ref{fig:channel_iPRA}, respectively, and compared against their classic variants. Even though the results are computed for 
the complete three-dimensional field, only two-dimensional cross sections are presented in the following. 
In figures \ref{fig:channel_iFTLE} and \ref{fig:channel_iPRA}, a $\left(y-z\right)$ cross-section located at $x=2 \pi h$ is shown.
The three dimensional visualisation of 
invariant manifolds poses a challenge on its own, which is object of current research
in computer visualisation {\color{red} XXX CITE XXX} and is not in the scope of the present study. 
The specific location of the cross section results in different local flow realisations, which however
always highlight similar turbulent structures known to populate turbulent channel flows. These are, for instance,
low-speed streaks, quasi-streamwise and hairpin vortices and packets thereof {\color{red} (Robinson 1991)}. The additional material
{\color{red} \textsf{Movie 3.mov}} and {\color{red} \textsf{Movie 4.mov}} show how figure \ref{fig:channel_iFTLE}(b-c) change throughout the 
channel length. 

\iffalse
\begin{figure}
  \centering
  \includegraphics[]{./Figures/velocity/mFTLE_inset.pdf}\\
  \includegraphics[]{./Figures/momentum/mFTLE_inset.pdf}\\
  \includegraphics[]{./Figures/vorticity/mFTLE_inset.pdf}
  \caption{Comparison between the instantaneous limit of (a) the classic FTLE, 
           (b) the active FTLE with respect to $\rho \mathbf{u}$ and (c) the 
           active FTLE with respect to $\bm{\omega}$ at $t=0$ in a cross-sectional
           plane at $x/h = 2\pi$.  }
  \label{fig:channel_iFTLE}
\end{figure}
\fi
\begin{figure}
  %\centering
  \includegraphics[]{./Figures/ChannelFlow/velocity/mFTLE.pdf}\\
  \includegraphics[]{./Figures/ChannelFlow/momentum/mFTLE.pdf}\\
  \includegraphics[]{./Figures/ChannelFlow/vorticity/mFTLE.pdf}\\
  \hfill\includegraphics[]{./Figures/ChannelFlow/velocity/inset.pdf}\hfill\includegraphics[]{./Figures/ChannelFlow/momentum/inset.pdf}\hfill\includegraphics[]{./Figures/ChannelFlow/vorticity/inset.pdf}\hfill
  \caption{Comparison between the instantaneous limit of (a,d) the classic FTLE, 
           (b,e) the active FTLE with respect to $\rho \mathbf{u}$ and (c,f) the 
           active FTLE with respect to $\bm{\omega}$ at $t=0$ in a cross-sectional
           plane at $x/h = 2\pi$. The panels (d-f) magnify the region denoted with a rectangle in panels (a-c).  }
  \label{fig:channel_iFTLE}
\end{figure}
%%%
\begin{figure}
  %\centering
  \includegraphics[]{./Figures/ChannelFlow/velocity/mPRA.pdf}\\
  \includegraphics[]{./Figures/ChannelFlow/momentum/mPRA.pdf}\\
  \includegraphics[]{./Figures/ChannelFlow/vorticity/mPRA.pdf}\\
  \hfill\includegraphics[]{./Figures/ChannelFlow/velocity/insetPRA.pdf}\hfill\includegraphics[]{./Figures/ChannelFlow/momentum/insetPRA.pdf}\hfill\includegraphics[]{./Figures/ChannelFlow/vorticity/insetPRA.pdf}\hfill
  \caption{Comparison between the instantaneous limit of (a,d) the classic PRA, 
           (b,e) the active PRA with respect to $\rho \mathbf{u}$ and (c,f) the 
           active PRA with respect to $\bm{\omega}$ at $t=0$ in a cross-sectional
           plane at $x/h = 2\pi$. The panels (d-f) magnify the region denoted with a rectangle in panels (a-c).}
  \label{fig:channel_iPRA}
\end{figure}

As already discussed in \S{\color{red}9},  
the active FTLE and PRA, thanks to the autonomous nature of the barrier 
equation {\color{red} (20)}, are capable to visually highlight
a broader range of structures compared to their classic variants. 
These structures are visible in figures \ref{fig:channel_iFTLE} and 
\ref{fig:channel_iPRA} as an abundance of invariant manifolds. Limiting to visual inspection, 
we recognise several open (or hyperbolic) barriers as ridges of the FTLE fields. 
Given the quasi-stramwise nature of turbulent 
structures in wall-bounded flows, vortical (or elliptic) barriers to transport 
are often observed in cross-sectional planes as FTLE ridges wrapping around closed regions, which are 
in turn confirmed as level sets of the corresponding PRA field. Example of such regions
are shown in the magnifications of panels (d-f) in figures \ref{fig:channel_iFTLE} and 
\ref{fig:channel_iPRA}. 


The results also reveal that large prominent FTLE ridges penetrate into and span the bulk flow region, sometimes
connecting the channel halves, as visible in \ref{fig:channel_iFTLE}(b) between $3 \leq z/h \leq 3.5$ and $0.3 \leq y/h \leq 1.5$.
Other regions, such as between $2 \leq z/h \leq 3$ and $0.5 \leq y/h \leq 1.5$ in the same figure, display practically no discernible barriers  
and are bounded by the envelopes of filamented open (hyperbolic)
transport barriers, which are finite-time generalizations of infinite-time
classic stable and unstable manifolds. Unlike in previous approaches,
however, these finite-time invariant manifolds are constructed here
as perfect barriers to active transport, rather than as Lagrangian
coherent structures acting as backbones of advected fluid-mass patterns
{\color{red} (Haller 2015)}. 



\begin{figure}
  \centering
  \includegraphics[]{./Figures/ChannelFlow/momentum/arrows.pdf}\includegraphics[]{./Figures/ChannelFlow/vorticity/arrows.pdf}\\
  \caption{Instantaneous active barriers of (a) $\rho \mathbf{u}$ and (b) $\bm{\omega}$ at $t=0$ in a cross-sectional
           plane located at $x/h = 2\pi$. The colormap shows the respective aFTLE fields, the vectors show the cross-sectional 
           components of the underlying active barrier field, while the red lines are level-set curves $\lambda_{2}^{+}(\mathbf{x},t)=-0.015$ 
           of the Eulerian vortex identification criterion proposed by {\color{red} Jeong et al. (1997)}.}
  \label{fig:ibfield}
\end{figure}
%%%

Figure \ref{fig:ibfield} shows the instantaneous active barrier vector field of (a) $\rho\mathbf{u}$ and (b) $\bm{\omega}$
superimposed to the respective aFTLEs already shown in figure \ref{fig:channel_iFTLE}(e-f).  
Level-set curves of the $\lambda_{2}(\mathbf{x},t)=-0.015$ field (Jeong \&
Hussein 1995), a common visualization tool for coherent vortical structures in 
wall-bounded turbulence, are also shown. The scalar
field  $\lambda_{2}(\mathbf{x},t)$  is defined as the instantaneous intermediate
eigenvalue of the tensor field $\mathbf{S}^{2}(\mathbf{x},t)+\mathbf{W}^{2}(\mathbf{x},t)$,
where \textbf{$\mathbf{S}$ }is the rate-of-strain tensor (the symmetric
part of the velocity gradient) and $\mathbf{W}$ is the spin tensor
(the skew-symmetric part of the velocity gradient). This choice follows the 
heuristic convention to select a $\lambda_{2}^{+}$
value slightly below the negative of the r.m.s. peak of $\lambda_{2}(\mathbf{x},t)$
across the channel (Jeong et al. 1997), which is approximately $0.0125$
in our case.


Compared to the classic material barriers shown in figure \ref{fig:channel_iFTLE}(d), we observe that 
the active barriers not only yield a remarkably more complex flow structure but also carry a 
completely different physical meaning. Since the active barriers minimise the diffusive transport of, in this case,
 linear momentum or vorticity, we find that the cross-sectional components of the active
barrier vector field $\mathbf{b}_t^t$ are parallel to the FTLE ridges. 
This indicates that the resultant force 
%In other words, for instance, the resultant force 
of the viscous stresses is tangential to instantaneous barriers of momentum. As noted previously, momentum barriers in $\left(y-z\right)$ cross-sections
can roll-up into spiral patterns or form closed surfaces. In regions where this occurs, 
figure \ref{fig:ibfield}(a) shows that closed level-set curves of $\lambda_2$, typically used as indicators for 
%associated with 
the presence of quasi-streamwise vortices, tend to be found. This suggests that
quasi streamwise vortices are associated to an instantaneous active barrier of linear momentum. 
Interestingly, we find that the circulation of the active momentum barrier field in such areas is of opposite sign than the one of the velocity field.  This indicates that viscous forces oppose the vortical motion that is observed in the analyzed snapshots.  %with respect to the 
%local the one of the velocity field. 
In addition, instantaneous barriers of vorticity tend to enter regions of closed  
momentum barriers or level-set curves of $\lambda_2$, thus highlighting regions in which vorticity diffuses into the vortex 
or is dissipated by viscosity. 

Despite some similarities it is important to note that there are practical and fundamental differences between the 
instantaneous momentum barriers and level-set surfaces of $\lambda_2$. On the fundamental side, we mention that 
the active barriers are objective, they have clear implications for the viscous transport of the active vector field and, most importantly, 
that they are extensible by definition to material barriers, thus accounting for the Lagrangian coherence of the barriers themselves. 
On the practical side, instantaneous active barriers do not require the convenient but arbitrary choice of a threshold and deliver information on the whole active
vector field. 

%%%
\iffalse


Here we choose
the level set defined by $\lambda_{2}^{+}(\mathbf{x},t)=-0.02$, with
the $+$ superscript referring to the usual scaling in wall units.
 In Fig. \ref{fig: 3D channel - Eulerian momentum barriers and lambda2},
we show a three-dimensional image of the Eulerian momentum barriers
in several cross sections, with certain level sets of the $\lambda_{2}^{+}$
parameter superimposed. The lower inset shows a portion of the flow
where the (frame and threshold-dependent) $\lambda_{2}^{+}$ surface
is locally consistent with some of the objectively defined tubular
barrier highlighted by the FTLE plot. The higher inset, however, shows
a flow region where none of the objective barrier surfaces are signaled
by $\lambda_{2}^{+}$ level sets. The latter barriers, therefore,
represent false negatives for barrier-detection via the $\lambda_{2}^{+}$
parameter.
\begin{figure}
	\begin{centering}
		\includegraphics[width=0.9\textwidth]{Figures/momentumBarrierShort.pdf}
		\par\end{centering}
	\caption{Intersections of instantaneous momentum barrier surfaces with three
		different planes at time $t=0$, highlighted by ridges of the FTLE
		field of the second equation in \eqref{eq:NS momentum barrier eq-1}.
		Some trajectories of this Eulerian barrier equation are also shown
		for reference (in cyan). Superimposed are the components of the instantaneous
		level set $\lambda_{2}^{+}(\mathbf{x},t)=-0.02$, which is traditionally
		used for vortex identification in turbulent channel flows. Instances
		of similarities (lower inset), false negatives (upper inset) and false
		positives suggested by the $\lambda_{2}^{+}$ level sets can be found.}\label{fig: 3D channel - Eulerian momentum barriers and lambda2}
\end{figure}


\noindent Figures \ref{fig: 3D channel - Eulerian vorticity barriers}-\ref{fig: 3D channel - Lagrangian vorticity barriers}
show the corresponding FTLE- and PRA-based visualizations of instantaneous
and material barriers to vorticity transport within the same two-dimensional
cross-section of the channel. The range for the streamline parametrization
$\mathbf{x}_{0}(s)$ of the barrier equations was $s\in[0,0.0001]$
for both the Eulerian and Lagrangian computations. This is significantly
shorter than the range we used to explore momentum barriers. The reason
is that the barrier equations for vorticity have right-hand sides
that are orders of magnitude larger due to the additional spatial
derivative involved in their definition. 

\noindent Figures \ref{fig: 3D channel - Eulerian vorticity barriers}-\ref{fig: 3D channel - Lagrangian vorticity barriers}
highlight structures that are similar, but not identical, to the momentum
barriers shown in Figs. \ref{fig: 3D channel - Eulerian momentum barriers}-\ref{fig: 3D channel - Lagrangian momentum barriers}.
The similarity is especially notable between the Lagrangian momentum
and vorticity barriers (lower subplots of Figs. \ref{fig: 3D channel - Lagrangian momentum barriers}
and \ref{fig: 3D channel - Lagrangian momentum barriers}), where
the Lagrangian averaging appears to compensate for the differences
arising from the different orders of spatial differentiations involved
in obtaining their Eulerian counterparts in the upper subplots in
the same figures. 
\begin{figure}
	\begin{centering}
		\includegraphics[width=0.85\textwidth]{Figures/2D_section_of_channel_Eulerian_vorticity_barriers.pdf}
		\par\end{centering}
	\caption{Time $t_{0}=0$ positions of instantaneous (Eulerian) barriers to
		vorticity transport, highlighted by the FTLE field (upper plot) and
		the PRA field (lower plot) of the momentum second barrier equation
		in \eqref{eq:NS momentum barrier eq-1}. FTLE values range within
		the interval $[0,3.5\times10^{4}]$ and PRA values range within the
		interval $[0,3.25].$ All other details are the same as for the instantaneous
		momentum barriers in Fig. \ref{fig: 3D channel - Eulerian momentum barriers}.}\label{fig: 3D channel - Eulerian vorticity barriers}
\end{figure}

\begin{figure}
	\begin{centering}
		\includegraphics[width=0.85\textwidth]{Figures/2D_section_of_channel_Lagrangian_vorticity_barriers.pdf}
		\par\end{centering}
	\caption{Same as Fig. \ref{fig: 3D channel - Lagrangian momentum barriers}
		but for material (Lagrangian) vorticity barriers.}\label{fig: 3D channel - Lagrangian vorticity barriers}
\end{figure}
Finally, in Fig. \ref{fig: 3D channel - Eulerian vorticity barriers and lambda2},
we highlight Eulerian vorticity barriers and compare them with the
same $\lambda_{2}^{+}$ level-sets that we have already shown in Fig.
\ref{fig: 3D channel - Eulerian momentum barriers and lambda2}. The
lower inset again shows a portion of the flow where the $\lambda_{2}^{+}$
surface is locally consistent with some of the objectively defined
tubular barriers to vorticity transport. The higher inset shows cases
of false positives for the detection of vorticity-transport barriers
via the $\lambda_{2}^{+}$ parameter.
\begin{figure}
	\begin{centering}
		\includegraphics[width=0.9\textwidth]{Figures/vorticityBarrierShort.pdf}
		\par\end{centering}
	\caption{Intersections of instantaneous vorticity barrier surfaces with three
		different planes at time $t=0$, highlighted by ridges of the FTLE
		field of the second equation in \eqref{eq:NS momentum barrier eq-1}.
		Some trajectories of this Eulerian barrier equation are also shown
		for reference (in cyan). Superimposed are the components of the instantaneous
		level set $\lambda_{2}^{+}(\mathbf{x},t)=-0.02$. Instances of similarities
		(lower inset), false positives (upper inset) and false negatives suggested
		by the $\lambda_{2}^{+}$ level-sets can be found.}\label{fig: 3D channel - Eulerian vorticity barriers and lambda2}
\end{figure}
\fi

% ==============================================================================
% ==============================================================================
\subsubsection{Material barriers to active transport} \label{sec:l3d}


\begin{figure}
  \centering
  \includegraphics[]{Figures/ChannelFlow/velocity.lagrangian/bFTLE750.pdf}
  \caption{Classic backward $\mathrm{FTLE}_0^{-3.75}\left(\mathbf{x}_0 \right)$ in a cross-sectional
           plane at $x/h = 2\pi$. The right panel magnifies the region denoted with a rectangle in the left panel. }
  \label{fig:bFTLE}
\end{figure}
Figure \ref{fig:bFTLE} shows attracting material surfaces as classic backward  $\mathrm{FTLE}_0^{-3.75}\left(\mathbf{x}_0 \right)$ at the same $\left(y-z\right)$ cross-section located at $x=2 \pi h$ discussed in \S\ref{sec:i3d}. The attracting material surfaces strikingly resemble the instantaneous barriers to linear momentum shown in figure \ref{fig:channel_iFTLE}(b,e) as $\mathrm{aFTLE}_{0,0}^{31}\left(\mathbf{x}_0, \rho\mathbf{u} \right)$. The close similarity between the two is not fully surprising. At the present low value of Reynolds number viscous effects dominate throughout a significant portion of the channel, and thus determine both the characteristics of the instantaneous momentum barriers and the finite-time dynamics of particle motion. The temporal horizon, over which the analogy between  $\mathrm{FTLE}_0^{-3.75}\left(\mathbf{x}_0 \right)$ and $\mathrm{aFTLE}_{0,0}^{31}\left(\mathbf{x}_0, \rho\mathbf{u} \right)$ is observed, is supposed to decrease with increasing Reynolds number, as the viscosity-dominated inner layer shrinks compared to the channel height. Whether the similarity holds at higher values of $Re$ is to be verified in later studies with high-$Re$ data. However, it is remarkable that the instantaneous momentum barriers, which are computed utilising a single flow snapshot, reproduce the same features of material surfaces obtained from a Lagrangian computation, which requires storing the temporal evolution of the flow. 

\begin{figure}
  %\centering
  \includegraphics[]{./Figures/ChannelFlow/velocity.lagrangian/fFTLE750.pdf}\\
  \includegraphics[]{./Figures/ChannelFlow/momentum.lagrangian/fFTLE750.pdf}\\
  \includegraphics[]{./Figures/ChannelFlow/vorticity.lagrangian/fFTLE750.pdf}\\
  \hfill\includegraphics[]{./Figures/ChannelFlow/velocity.lagrangian/inset750.pdf}\hfill\includegraphics[]{./Figures/ChannelFlow/momentum.lagrangian/inset750.pdf}\hfill\includegraphics[]{./Figures/ChannelFlow/vorticity.lagrangian/inset750.pdf}\hfill
  \caption{ Comparison between (a,d) the classic FTLE, 
            (b,e) the active FTLE with respect to $\rho \mathbf{u}$ and (c,f) the 
            active FTLE with respect to $\bm{\omega}$ in a cross-sectional
            plane at $x/h = 2\pi$. The integration interval is for all cases between $t_0=0$ and $t_1=3.75$. 
            The panels (d-f) magnify the region denoted with a rectangle in panels (a-c). }
  \label{fig:channel_lFTLE}
\end{figure}
\begin{figure}
  %\centering
  \includegraphics[]{./Figures/ChannelFlow/velocity.lagrangian/fPRA750.pdf}\\
  \includegraphics[]{./Figures/ChannelFlow/momentum.lagrangian/fPRA750.pdf}\\
  \includegraphics[]{./Figures/ChannelFlow/vorticity.lagrangian/fPRA750.pdf}\\
  \hfill\includegraphics[]{./Figures/ChannelFlow/velocity.lagrangian/insetPRA750.pdf}\hfill\includegraphics[]{./Figures/ChannelFlow/momentum.lagrangian/insetPRA750.pdf}\hfill\includegraphics[]{./Figures/ChannelFlow/vorticity.lagrangian/insetPRA750.pdf}\hfill
  \caption{ Comparison between (a,d) the classic PRA, 
            (b,e) the active PRA with respect to $\rho \mathbf{u}$ and (c,f) the 
            active PRA with respect to $\bm{\omega}$ in a cross-sectional
            plane at $x/h = 2\pi$. The integration interval is for all cases between $t_0=0$ and $t_1=3.75$. 
            The panels (d-f) magnify the region denoted with a rectangle in panels (a-c).}
  \label{fig:channel_lPRA}
\end{figure}
Figures \ref{fig:channel_lFTLE} and \ref{fig:channel_lPRA} show aFTLE and aPRA, respectively, in a $\left(y-z\right)$ cross-section located at $x=2 \pi h$ and compare them against their classic variants. The integration interval is for all cases between $t_0=0$ and $t_1=3.75$. The figures clearly show that some features of the instantaneous active barriers discussed in \S\ref{sec:i3d}, such as the spiralling or closed patterns of $\mathrm{aFTLE}_{0,0}^{31}\left(\mathbf{x}, \rho \mathbf{u} \right)$, do have a material character, since they persist almost unchanged over the temporal interval which we have considered. Examples are shown in the magnification of figures \ref{fig:channel_lFTLE}(e) and \ref{fig:channel_lPRA}(e). In the vicinity of the wall, characterised by the strong intermittent turbulent events rapidly evolving with the viscous timescale, less detail is visible in the barriers, due to the lack of material coherence for the considered time frame. %The comparison against the classic LCS, shown in figures \ref{fig:channel_lFTLE}(a,e) and \ref{fig:channel_lPRA}(a,e), allows to analyse, whether LCSs play a role in inhibiting the diffusive transport of momentum or vorticity. 


\begin{figure}
  \centering
  \includegraphics[]{./Figures/ChannelFlow/momentum.lagrangian/arrows.pdf}\includegraphics[]{./Figures/ChannelFlow/vorticity.lagrangian/arrows.pdf}\\
  \caption{Material active barriers of (a) $\rho \mathbf{u}$ and (b) $\bm{\omega}$ at $t=0$ in a cross-sectional
           plane located at $x/h = 2\pi$ and for an integration interval between $t_0=0$ and $t_1=3.75$. 
           The colormap shows the respective aFTLE fields, the vectors show the cross-sectional 
           components of the underlying active barrier field, while the red lines are level-set curves $\lambda_{2}^{+}(\mathbf{x},t)=-0.015$ 
           of the Eulerian vortex identification criterion proposed by {\color{red} Jeong et al. (1997)} at the instant $t_0=0$.}
  \label{fig:lbfield}
\end{figure}
Figure \ref{fig:lbfield} shows the material active barrier vector field of (a) $\rho\mathbf{u}$ and (b) $\bm{\omega}$
superimposed to the respective aFTLEs already shown in figure \ref{fig:channel_lFTLE}(e-f).  
Level-set curves of the $\lambda_{2}(\mathbf{x},t)=-0.015$ field at the temporal instant $t=t_0=0$ are also shown. It is confirmed that with the present definition of active barriers, the active vector field is tangent to the detected barriers visualised here as aFTLE ridges, in a temporally-averaged sense. Figure \ref{fig:lbfield}(a) shows that closed $\mathrm{aFTLE}_{t_0,t_1}^{s}\left(\mathbf{x}_0, \rho\mathbf{u} \right)$ ridges can be in some instances close to level-set curves of the $\lambda_{2}$ criterion, as for instance at $(y/h, z/h) \approx (0.15,2.9)$ and $(0.55,3.3)$. In this sense, the material momentum barriers can be utilised as means to objectively identify vortical structures which play a role in inhibiting momentum transport and preserve material coherence over the considered time frame, without resorting to any arbitrary level-set. 

